Automatic Differentiation-based Full Waveform Inversion with Flexible Workflows

Full waveform inversion (FWI) is able to construct high-resolution subsurface models by iteratively minimizing discrepancies between observed and simulated seismic data. However, its implementation can be rather involved for complex wave equations, objective functions, or regularization. Recently, automatic differentiation (AD) has proven to be effective in simplifying solutions of various inverse problems, including FWI. In this study, we present an open-source AD-based FWI framework (ADFWI), which is designed to simplify the design, development, and evaluation of novel approaches in FWI with flexibility. The AD-based framework not only includes forword modeling and associated gradient computations for wave equations in various types of media from isotropic acoustic to vertically or horizontally transverse isotropic elastic, but also incorporates a suite of objective functions, regularization techniques, and optimization algorithms. By leveraging state-of-the-art AD, objective functions such as soft dynamic time warping and Wasserstein distance, which are difficult to apply in traditional FWI are also easily integrated into ADFWI. In addition, ADFWI is integrated with deep learning for implicit model reparameterization via neural networks, which not only introduces learned regularization but also allows rapid estimation of uncertainty through dropout. To manage high memory demands in large-scale inversion associated with AD, the proposed framework adopts strategies such as mini-batch and checkpointing. Through comprehensive evaluations, we demonstrate the novelty, practicality and robustness of ADFWI, which can be used to address challenges in FWI and as a workbench for prompt experiments and the development of new inversion strategies.

==> cover_letter.tex <==
Dear Editors,

I am pleased to submit our manuscript, titled “Automatic Differentiation-based Full Waveform Inversion with Flexible Workflows”, for consideration in JGR Machine Learning and Computation. This manuscript has not been submitted for publication elsewhere, nor is it under consideration by any other journal.

In this work, we introduce ADFWI, an open-source, automatic differentiation-based full waveform inversion (FWI) framework. The objective of our framework is to facilitate the development, testing and implementation of advanced FWI strategies in a flexible and efficient manner. By integrating state-of-the-art AD capabilities, ADFWI allows the straightforward incorporation of complex wave equations (e.g. vertically transverse isotropy and horizontal transverse isotropic medium), objective functions (e.g. soft dynamic time warping and Wasserstein distance) and regularization techniques, which have historically been challenging to apply in FWI workflows. Furthermore, our framework supports neural network-based implicit model reparameterisation, enabling learned regularisation and uncertainty quantification through dropout.

Recognizing the inherent challenges associated with AD, such as high memory demands in large-scale inversions, ADFWI provides practical strategies, including mini-batch processing and checkpointing, to mitigate these issues. Its versatility and practicality are demonstrated through extensive evaluations, showcasing its robustness and adaptability for addressing FWI challenges while serving as a platform for experimenting with innovative inversion strategies.

We believe that this manuscript will be of interest to the readership of JGR Machine Learning and Computational, particularly to those engaged in developing computational tools for geophysical applications or exploring advanced machine learning methods in inverse problems. The results we present contribute to a growing body of work leveraging automatic differentiation and deep learning for high-resolution subsurface imaging, offering a flexible framework for rapid experimentation and innovation.

Thank you for considering our submission. We look forward to the opportunity to share this work with the scientific community and are available to provide additional information or address any questions related to the manuscript.

Best Regards,

Junlun Li
School of Earth and Space Sciences
University of Science and Technology of China 
96 Jinzhai Road, Hefei, 230026, Anhui, China. 
86-551-63603533
lijunlun@ustc.edu.cn
